Gaussian Process Regression and Classification under Mathematical Constraints with Learning Guarantees

We introduce constrained Gaussian process (CGP), a Gaussian process model for random functions that allows easy placement of mathematical constrains (e.g., non-negativity, monotonicity, etc) on its sample functions. CGP comes with closed-form probability density function (PDF), and has the attractive feature that its posterior distributions for regression and classification are again CGPs with closed-form expressions. Furthermore, we show that CGP inherents the optimal theoretical properties of the Gaussian process, e.g. rates of posterior contraction, due to the fact that CGP is an Gaussian process with a more efficient model space.

==> preamble/author_article.tex <==
%% Here are the title, author names and addresses
\title{Constrained Gaussian Process for Regression, Classification and Distribution Estimation}

\author{Jeremiah Z. Liu\thanks{zhl112@mail.harvard.edu.}}
\affil{Department of Biostatistics, Harvard University, Boston, MA, USA.}
\date{}


==> preamble/packages_article.tex <==
\makeatletter
\providecommand{\@LN}[2]{}
\makeatother

\usepackage[margin=1in]{geometry}
\usepackage{times}
\usepackage{graphicx,psfrag,epsf}
\usepackage{enumerate}
\usepackage{natbib}
\usepackage{url} % not crucial - just used below for the URL 
\usepackage{setspace}
\setstretch{1.8}

%\pdfminorversion=4
% NOTE: To produce blinded version, replace "0" with "1" below.
\newcommand{\blind}{0}

\newlength\tindent
\setlength{\tindent}{\parindent}
\setlength{\parindent}{0pt}
\renewcommand{\indent}{\hspace*{\tindent}}

% DON'T change margins - should be 1 inch all around.
% \addtolength{\oddsidemargin}{-.5in}%
% \addtolength{\evensidemargin}{-.5in}%
% \addtolength{\textwidth}{1in}%
% \addtolength{\textheight}{-.3in}%
% \addtolength{\topmargin}{-.8in}%

%  If your system does not have the AMS fonts version 2.0 installed, then
%  remove the useAMS option.
%
%  useAMS allows you to obtain upright Greek characters.
%  e.g. \umu, \upi etc.  See the section on "Upright Greek characters" in
%  this guide for further information.
%
%  If you are using AMS 2.0 fonts, bold math letters/symbols are available
%  at a larger range of sizes for NFSS release 1 and 2 (using \boldmath or
%  preferably \bmath).
% 
%  Other options are described in the user guide. Here are a few:
% 
%  -  If you use Patrick Daly's natbib  to cross-reference your 
%     bibliography entries, use the usenatbib option
%
%  -  If you use \includegraphics (graphicx package) for importing graphics
%     into your figures, use the usegraphicx option
% 
%  If you wish to typeset the paper in Times font (if you do not have the
%  PostScript Type 1 Computer Modern fonts you will need to do this to get
%  smoother fonts in a PDF file) then uncomment the next line
%  \usepackage{Times}

% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[final]{nips_2017}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{comment}      % comment
\usepackage{multirow}

%
\usepackage{graphicx}
\usepackage{subcaption}


% 
\usepackage{amsmath}
\usepackage{amssymb, mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}
\usepackage{amsthm}

%
\usepackage{algorithm}
\usepackage{algpseudocode}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

%
\usepackage{authblk}

%
\usepackage{color} % pre-req for below macros
\usepackage{xcolor}
\usepackage{"./macro/GrandMacros"}
\usepackage{"./macro/Macro_BIO235"}

% theorem
\newtheoremstyle{break}
  {\topsep}{\topsep}%
  {\itshape}{}%
  {\bfseries}{}%
  {\newline}{}%
  
\theoremstyle{break}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}


==> sections/cgp.tex <==
\section{Constrained Gaussian Process}
\label{sec:cgp}

In this section we introduce the \gls{CGP}, a \gls{GP} model for random functions that equips its sample paths with suitable mathematical constrains. %In Section \ref{sec:model}, we use \gls{CGP} to model the \gls{BNE}'s \gls{CDF} so the posterior respects the boundedness and monotonicity of a distribution function. 
\gls{CGP} has closed-form \gls{PDF} and \gls{MGF}, and comes with an intuitive geometric interpretation as assigning probability mass to the intersection between multiple convex sets. The distinguishing feature of \gls{CGP} is that its posterior distribution for regression and classification are again \gls{CGP}. Furthermore, \gls{CGP} inherents the optimal theoretical properties of the Gaussian process, e.g. universal approximation property for continuous functions with a compact support \citep{micchelli_learning_2005} and optimal rates of posterior contraction \citep{vaart_rates_2008}, due to the fact that \gls{CGP} is simply an Gaussian process with a restricted sample space.

Conceptually, the goal of a constrained Gaussian process (CGP) is to place mathematical constraints $\Csc$ on the sample paths $g$ of a Gaussian process, such that $g \in \Csc$. Operationally, $\Csc$ is defined through a system of $k$ linear constraints characterized by matrices $\bA_{k \times 1}$ and $\bb_{k \times 1}$, e.g.:
\begin{alignat*}{3}
    \mbox{sample} \quad & g \sim GP(0, k) \\
    \mbox{subject to} \quad & g \in \Csc 
    \qquad \qquad \mbox{where} \quad
    \Csc = \{g | \bA g + \bb \geq 0\}.
\end{alignat*}
For example, an inequality constraint $\Csc=\{g | g \geq 0 \}$ can be written as $\bA = 1, \bb = 0$, and a boundedness constraint $\Csc=\{g | 1 \geq g \geq 0 \}=\{g | g \geq 0,  1 - g \geq 0 \}$ can be written as $\bA = [1, -1]^\top, \bb = [0, 1]^\top$. Notice that since $g$ is a random variable, the constraint $\Csc$ is a random event with distribution $f(\Csc|g)$. Consequently, \gls{CGP} imposes constraints $\Csc$ on a Gaussian process by augmenting the original distribution of a \gls{GP} $f(g)$ with the additional likelihood term $P(\Csc|g)$.

As a result, given constraints $\Csc$ and a standard \gls{GP} with mean function $\mu$ and kernel function $k$, the likelihood function of \gls{CGP} is defined to be:
\begin{align}
    f(g|\Csc) \propto f(\Csc|g)f(g),
    \label{eq:cgp_lkhd}
\end{align}
where $f(g) = GP(g | \mu, k)$ is the likelihood for the standard \gls{GP}. $f(\Csc|g)$ is designed such that it assigns near zero probability to $g$'s that violates $\Csc$, and assign high probability otherwise. In this work, we use the Probit function (i.e. the \gls{CDF} of a standard Gaussian distribution) to represent the likelihood functions for each individual constraint in $\Csc$, and assume the $k$ constraints are independent conditional on $G$. As a result, $P(\Csc|G)$ is the \gls{CDF} of a standard multivariate Gaussian distribution:
\begin{align*}
    f(\Csc|g) \propto \Phi(\bA g + \bb | \bmu=\bzero, \bSigma=\bI)
\end{align*}
where we denote $\Phi(.|\bmu, \bSigma)$ and $\phi(.|\bmu, \bSigma)$ to be the \gls{CDF} and \gls{PDF} of a Gaussian distribution with mean $\bmu$ and covariance $\bSigma$. To keep the notations uncluttered, in the rest of this section we will drop the terms $\bmu$ and $\bSigma$ unless they are different from the default values $\bmu=\bzero$ and $\bSigma=\bI$. Consequently, conditional on the function input $\bz$, the  likelihood function of \gls{CGP} for $\bg = g(\bz)$ is:
\begin{align}
    f(\bg|\Csc) 
    &\propto f(\Csc|\bg) * f(\bg), \nonumber \\
    &\propto \Phi(\bA \bg + \bb) * \phi(\bg |\bu,  \bK),
    \label{eq:cgp_cond_lkhd}
\end{align}
where $\bu$ and $\bK$ are the mean vector and the kernel matrix of the standard GP $f(g) = GP(g | \mu, k)$ evaluated at  $\bz$.

\subsection{\gls{PDF}, \gls{MGF} and Moments}
Given constraints $\Csc = \{ g | \bA g + \bb \geq 0\}$ and a standard Gaussian process $GP(\mu, k)$, denote the Constrained Gaussian Process (CGP) as $CGP(\mu, k, \Csc)$. For $g \sim CGP(\Csc, \mu, k)$, given input $\bz$, the \gls{PDF} of $\bg = g(\bz)$ is:
\begin{align}
    f(\bg |\bu, \bK, \Csc) = 
    \frac{\phi(\bg |\bu,  \bK) * \Phi(\bA \bg + \bb)}{C}
    \quad \mbox{where} \quad 
    C = \Phi(\bA\bu + \bb|\Sigma = \bI + \bA\bK\bA^\top)
    \label{eq:cpg_pdf}
\end{align}
and the \gls{MGF} of $CGP(\Csc, \mu, k)$ is:
\begin{align}
    M_{\bg}(\bt) 
    %&= E(exp(\bt^\top\bg)|\Csc, \bu, \bK)  \nonumber\\
    &= exp(\bu^\top\bt + \frac{1}{2} \bt^\top \bK \bt ) * 
    \frac{
    \Phi(\bA\bu + \bb + \bA\bK\bt |\Sigma = \bI + \bA\bK\bA^\top)}{
    \Phi(\bA\bu + \bb|\Sigma = \bI + \bA\bK\bA^\top)}
    \label{eq:cpg_mgf}
\end{align}
where recall $\Phi(.|\bmu, \bSigma)$ and $\phi(.|\bmu, \bSigma)$ are the \gls{CDF} and \gls{PDF} of a Gaussian distribution with mean $\bmu$ and covariance $\bSigma$.
\begin{proof} 
See Section \ref{sec:cgp_pdf_mgf_proof}
\end{proof}

As a result, the moments of $CGP(\Csc, \mu, k)$ can be derived by taking derivatives with respect to (\ref{eq:cpg_mgf}). In particular, the expression for the mean of CGP is
\begin{align}
    E(\bg|\bu, \bK, \Csc) 
    &=
    \bu + 
    \bK\bA^\top (\bI + \bA\bK\bA^\top)^{-1}
    E(\bb'| \bb' \geq -\bb, \Sigma=\bI + \bA\bK\bA^\top)
    \label{eq:cgp_mean}
\end{align}
In particular, the second term in (\ref{eq:cgp_mean}) corrects the original mean vector $\bmu$ with respect to the constraints such that $\bA E(\bg |\bu, \bK, \Csc) + \bb \geq 0$.
\begin{proof} 
See Section \ref{sec:cgp_pdf_mgf_proof}
\end{proof}

\subsection{Posterior Distribution for Regression and Classification}
An important feature of \gls{CGP} is that the posterior distributions of $\bg$ in regression and classification have closed forms. Specifically, assuming $g \sim CGP(\mu, k, \Csc)$, for a regression model $y_i \stackrel{indep}{\sim} Normal(g(\bz_i), \sigma^2)$, the posterior distribution of $\bg$ is again a constrained Gaussian process $CGP(\mu', k', \Csc')$ with parameters:
\begin{align*}
%    f(\bg |\Csc, \bu, \bK, \by) &= 
%    \frac{\phi(\bg |\bmu',  \Sigma') * \Phi(\bA \bg + \bb)}{
%    \Phi(\bA\bmu' + \bb|\Sigma = \bI + \bA\bSigma'\bA^\top)}
%    \qquad \mbox{where} \quad 
%    \label{eq:cpg_pdf_posterior}
%    \\
    \bmu' &= \bu + \bK(\bK + \sigma^2\bI)^{-1}(\by - \bu), 
    \quad 
    \bK' = \bK - \bK(\bK + \sigma^2\bI)^{-1}\bK,
    \quad 
    \Csc' = \Csc,
\end{align*}
and the predictive distribution for a new observation $\bz^*$ also follows a constrained Gaussian process $CGP(\mu^*, k^*, \Csc^*)$ with parameters:
\begin{align*}
\bmu^* &= u(\bz^*) + k(\bz^*, \bz)(\bK + \sigma^2\bI)^{-1}(\by - \bu),\\
\bK^* &= k(\bz^*, \bz^*) -  k(\bz^*, \bz)(\bK + \sigma^2\bI)^{-1}k(\bz, \bz^*),\\
\Csc^* &= \Csc.
\end{align*}
\begin{proof}
See Section \ref{sec:cgp_pdf_posterior_proof}
\end{proof}

For a classification model under the Probit link function $y_i \stackrel{indep}{\sim} Bernoulli(p_i), p_i = \Phi(g(\bz_i))$, the posterior distribution of $\bg$ is also a constrained Gaussian process $CGP(\mu', k', \Csc')$ but with modified constraint $\Csc'$:
\begin{align*}
    \bmu' = \bu, 
    \qquad 
    \bK' = \bK, 
    \qquad 
    \Csc' = \Bigg\{ \bg \Big|
    \begin{bmatrix} \bA \\ \bD \end{bmatrix} \bg + \begin{bmatrix} \bb \\ \bzero \end{bmatrix} \geq 0
    \Bigg\}
\end{align*}
where $\bD = diag(2 * \by - 1)$ is a diagonal matrix of $\pm 1$'s corresponding to the observations. Notice that the $\bD\bg$ term in $\Phi$ can be interpreted as imposing addition data-based constraints to $g(\bz_i)$, i.e.  $g(\bz_i) \geq 0$ when $y_i = 1$ and $g(\bz_i) \leq 0$ when $y_i = 0$, such that during estimation,  $g(\bz_i)$ is pushed toward positive/negative values depending on the value of the observation $y_i$. The predictive distribution for $g$ at new location $\bz^*$ is also a constrained GP $CGP(\mu^*, k^*, \Csc^*)$, with parameters:
\begin{align*}
\bmu^* &= u(\bz^*) + k(\bz^*, \bz)\bK^{-1}(\by - \bu),\\
\bK^* &= k(\bz^*, \bz^*) -  k(\bz^*, \bz)\bK^{-1}k(\bz, \bz^*),\\
\Csc^* &= \Bigg\{ \bg \Big|
        \begin{bmatrix} \bA \\ \bD \end{bmatrix} \bg + 
        \begin{bmatrix} \bb \\ \bzero \end{bmatrix} \geq 0
        \Bigg\}
\end{align*}
\begin{proof}
See Section \ref{sec:cgp_pdf_posterior_proof}
\end{proof}
%\input{"./sections/proof/cgp_posterior"}

==> sections/distribution.tex <==
Given constraints $\Csc = \{ g | \bA g + \bb \geq 0\}$ and a standard Gaussian process $GP(\mu, k)$, denote the Constrained Gaussian Process (CGP) as $CGP(\mu, k, \Csc)$. For $g \sim CGP(\Csc, \mu, k)$, given input $\bz$, the \gls{PDF} of $\bg = g(\bz)$ is:
\begin{align}
    f(\bg |\bu, \bK, \Csc) = 
    \frac{\phi(\bg |\bu,  \bK) * \Phi(\bA \bg + \bb)}{C}
    \quad \mbox{where} \quad 
    C = \Phi(\bA\bu + \bb|\Sigma = \bI + \bA\bK\bA^\top)
    \label{eq:cpg_pdf}
\end{align}
and the \gls{MGF} of $CGP(\Csc, \mu, k)$ is:
\begin{align}
    M_{\bg}(\bt) 
    %&= E(exp(\bt^\top\bg)|\Csc, \bu, \bK)  \nonumber\\
    &= exp(\bu^\top\bt + \frac{1}{2} \bt^\top \bK \bt ) * 
    \frac{
    \Phi(\bA\bu + \bb + \bA\bK\bt |\Sigma = \bI + \bA\bK\bA^\top)}{
    \Phi(\bA\bu + \bb|\Sigma = \bI + \bA\bK\bA^\top)}
    \label{eq:cpg_mgf}
\end{align}
where recall $\Phi(.|\bmu, \bSigma)$ and $\phi(.|\bmu, \bSigma)$ are the \gls{CDF} and \gls{PDF} of a Gaussian distribution with mean $\bmu$ and covariance $\bSigma$.

\jzl{see if we can derive a even more interpretable form for mean.}
As a result, we can derive the moments of $CGP(\Csc, \mu, k)$ by taking derivatives with respect to (\ref{eq:cpg_mgf}). In particular, the expression for the mean of CGP is
\begin{align}
    E(\bg|\bu, \bK, \Csc) 
    &=
    \bu + 
    \bK\bA^\top (\bI + \bA\bK\bA^\top)^{-1}
    E(\bb'| \bb' \geq -\bb, \Sigma=\bI + \bA\bK\bA^\top)
    \label{eq:cgp_mean}
\end{align}
In particular, the second term in (\ref{eq:cgp_mean}) corrects the original mean vector $\bmu$ with respect to the constraints such that $\bA E(\bg |\bu, \bK, \Csc) + \bb \geq 0$.

\jzl{maybe also derive variance.}
\begin{proof} 
See Section \ref{sec:cgp_pdf_mgf_proof}
\end{proof}



==> sections/idea.tex <==
Conceptually, the goal of a constrained Gaussian process (CGP) is to place mathematical constraints $\Csc$ on the sample paths $g$ of a Gaussian process, such that $g \in \Csc$. Operationally, $\Csc$ is defined through a system of $k$ linear constraints characterized by matrices $\bA_{k \times 1}$ and $\bb_{k \times 1}$, e.g.:
\begin{alignat*}{3}
    \mbox{sample} \quad & g \sim GP(0, k) \\
    \mbox{subject to} \quad & g \in \Csc 
    \qquad \qquad \mbox{where} \quad
    \Csc = \{g | \bA g + \bb \geq 0\}.
\end{alignat*}
For example, an inequality constraint $\Csc=\{g | g \geq 0 \}$ can be written as $\bA = 1, \bb = 0$, and a boundedness constraint $\Csc=\{g | 1 \geq g \geq 0 \}=\{g | g \geq 0,  1 - g \geq 0 \}$ can be written as $\bA = [1, -1]^\top, \bb = [0, 1]^\top$. Notice that since $g$ is a random variable, the constraint $\Csc$ is a random event with distribution $f(\Csc|g)$. Consequently, \gls{CGP} imposes constraints $\Csc$ on a Gaussian process by augmenting the original distribution of a \gls{GP} $f(g)$ with the additional likelihood term $P(\Csc|g)$.

As a result, given constraints $\Csc$ and a standard \gls{GP} with mean function $\mu$ and kernel function $k$, the likelihood function of \gls{CGP} is defined to be:
\begin{align}
    f(g|\Csc) \propto f(\Csc|g)f(g),
    \label{eq:cgp_lkhd}
\end{align}
where $f(g) = GP(g | \mu, k)$ is the likelihood for the standard \gls{GP}. $f(\Csc|g)$ is designed such that it assigns near zero probability to $g$'s that violates $\Csc$, and assign high probability otherwise. In this work, we use the Probit function (i.e. the \gls{CDF} of a standard Gaussian distribution) to represent the likelihood functions for each individual constraint in $\Csc$, and assume the $k$ constraints are independent conditional on $G$. As a result, $P(\Csc|G)$ is the \gls{CDF} of a standard multivariate Gaussian distribution:
\begin{align*}
    f(\Csc|g) \propto \Phi(\bA g + \bb | \bmu=\bzero, \bSigma=\bI)
\end{align*}
where we denote $\Phi(.|\bmu, \bSigma)$ and $\phi(.|\bmu, \bSigma)$ to be the \gls{CDF} and \gls{PDF} of a Gaussian distribution with mean $\bmu$ and covariance $\bSigma$. To keep the notations uncluttered, we will drop the terms $\bmu$ and $\bSigma$ unless they are different from the default values $\bmu=\bzero$ and $\bSigma=\bI$. Consequently, conditional on the function input $\bz$, the  likelihood function of \gls{CGP} for $\bg = g(\bz)$ is:
\begin{align}
    f(\bg|\Csc) 
    &\propto f(\Csc|\bg) * f(\bg), \nonumber \\
    &\propto \Phi(\bA \bg + \bb) * \phi(\bg |\bu,  \bK),
    \label{eq:cgp_cond_lkhd}
\end{align}
where $\bu$ and $\bK$ are the mean vector and the kernel matrix of the standard GP $f(g) = GP(g | \mu, k)$ evaluated at  $\bz$.
\jzl{add geometric interpretation}


==> sections/posterior.tex <==
An important feature of \gls{CGP} is that the posterior distributions of $\bg$ in regression and classification have closed forms. Specifically, assuming $g \sim CGP(\mu, k, \Csc)$, for a regression model $y_i \stackrel{indep}{\sim} Normal(g(\bz_i), \sigma^2)$, the posterior distribution of $\bg$ is again a constrained Gaussian process $CGP(\mu', k', \Csc')$ with parameters:
\begin{align*}
%    f(\bg |\Csc, \bu, \bK, \by) &= 
%    \frac{\phi(\bg |\bmu',  \Sigma') * \Phi(\bA \bg + \bb)}{
%    \Phi(\bA\bmu' + \bb|\Sigma = \bI + \bA\bSigma'\bA^\top)}
%    \qquad \mbox{where} \quad 
%    \label{eq:cpg_pdf_posterior}
%    \\
    \bmu' &= \bu + \bK(\bK + \sigma^2\bI)^{-1}(\by - \bu), 
    \quad 
    \bK' = \bK - \bK(\bK + \sigma^2\bI)^{-1}\bK,
    \quad 
    \Csc' = \Csc,
\end{align*}
and the predictive distribution for a new observation $\bz^*$ also follows a constrained Gaussian process $CGP(\mu^*, k^*, \Csc^*)$ with parameters:
\begin{align*}
\bmu^* &= u(\bz^*) + k(\bz^*, \bz)(\bK + \sigma^2\bI)^{-1}(\by - \bu),\\
\bK^* &= k(\bz^*, \bz^*) -  k(\bz^*, \bz)(\bK + \sigma^2\bI)^{-1}k(\bz, \bz^*),\\
\Csc^* &= \Csc.
\end{align*}

For a classification model under the Probit link function $y_i \stackrel{indep}{\sim} Bernoulli(p_i)$ where $p_i = \Phi(g(\bz_i))$, the posterior distribution of $\bg$ is also a constrained Gaussian process $CGP(\mu', k', \Csc')$ with modified constraint $\Csc'$:
\begin{align*}
    \bmu' = \bu, 
    \qquad 
    \bK' = \bK, 
    \qquad 
    \Csc' = \Bigg\{ \bg \Big|
    \begin{bmatrix} \bA \\ \bD \end{bmatrix} \bg + \begin{bmatrix} \bb \\ \bzero \end{bmatrix} \geq 0
    \Bigg\}
\end{align*}
where $\bD = diag(2 * \by - 1)$ is a diagonal matrix of $\pm 1$'s corresponding to the observations. Notice that the $\bD\bg$ term in $\Phi$ can be interpreted as imposing addition data-based constraints to $g(\bz_i)$, i.e.  $g(\bz_i) \geq 0$ when $y_i = 1$ and $g(\bz_i) \leq 0$ otherwise, such that during estimation,  $g(\bz_i)$ is pushed toward positive/negative values depending on the value of the observation $y_i$. The predictive distribution for $g$ at new location $\bz^*$ is also a constrained GP $CGP(\mu^*, k^*, \Csc^*)$, with parameters:
\begin{align*}
\bmu^* &= u(\bz^*) + k(\bz^*, \bz)\bK^{-1}(\by - \bu),\\
\bK^* &= k(\bz^*, \bz^*) -  k(\bz^*, \bz)\bK^{-1}k(\bz, \bz^*),\\
\Csc^* &= \Bigg\{ \bg \Big|
        \begin{bmatrix} \bA \\ \bD \end{bmatrix} \bg + 
        \begin{bmatrix} \bb \\ \bzero \end{bmatrix} \geq 0
        \Bigg\}
\end{align*}
\begin{proof}
See Section \ref{sec:cgp_pdf_posterior_proof}
\end{proof}
\jzl{also discuss prior centering. e.g. using $\Phi^{-1}_{\bSigma}$ which can be computed using Monte Carlo}



==> sections/proof/bne_accuracy.tex <==
Theorem \ref{thm:accuracy_rmse} is a special case of Theorem \ref{thm:accuracy} when the accuracy measure is \gls{MSE}. We present Theorem \ref{thm:accuracy} below. 

\begin{theorem}[Calibration Preserves Accuracy, General Loss]
Denote $F_0 \in \Fsc$ the uncalibrated predictive CDF, and $F=G \circ F_0 \in \Fsc$ the calibrated predictive CDF. 
Given observations $\{y_i, \bx_i\}_{i=1}^N$, we denote:
\begin{enumerate}
\item $\bbL(Y,F) = \frac{1}{N} \sum_{i=1}^N L(y_i, F(Y|\bX=\bx_i))$ with respect to a accuracy measure function $L: \Ysc \times \Fsc \rightarrow \real$ that is bounded and proper, i.e.:
\begin{enumerate}
\item \textbf{Bounded}: There exists positive constant $B<\infty$ such that $L(y, F) < B \quad \forall y \in \Ysc, F \in \Fsc$. Furthermore, for $F, F' \in \Fsc$ such that $\int_{\Ysc} \Big|F(t) - F'(t)\Big| dt < \epsilon$, we have: 
$$\int_{\Ysc} \Big|L(y, F') - L(y, F)\Big| dy < B\epsilon.$$
\item \textbf{Proper}: $\bbL(Y, F)$ is minimized by the true CDF $\Fbb$, i.e. $\bbL(Y, \Fbb) \leq \bbL(Y, F) \quad \forall F \in \Fsc$.
\end{enumerate}
\item $\bbC(Y, \hat{F})$ the empirical calibration loss defined as:
\begin{align*}
\bbC(Y, \hat{F}) &= \int_{\Ysc}
\frac{1}{N}\sum_{i=1}^n 
\Big| \bbI(y_i < t|\bx_i) - F(t|\bx_i) \Big| dt
\end{align*}
\end{enumerate}
Furthermore, we assume that $\hat{F}$ is $\epsilon_n$-calibrated \citep{abernethy_blackwell_2011}, i.e. $\underset{n \rightarrow \infty}{limsup}  \;\bbC(Y, \hat{F}) \leq \epsilon_n$ for some $\epsilon_n > 0$. 

Then the excess error of the calibrated CDF $\hat{F}$ with respect to the uncalibrated CDF $\hat{F}_0$ in terms of $\bbL$ is bounded by $\bbC$, i.e.
\begin{align*}
\bbL(Y, \hat{F}) - \bbL(Y, \hat{F}_0) \leq 2B * \bbC(Y, \hat{F}) + (B + 1)*\epsilon_n
\end{align*}
Morever, since $\hat{F}$ is $\epsilon_n$-calibrated:
\begin{align}
\underset{n \rightarrow \infty}{limsup} \Big[
\bbL(Y, \hat{F}) - \bbL(Y, \hat{F}_0) 
\Big] \leq (3B + 1)*\epsilon_n
\label{eq:excess_risk}
\end{align}
\label{thm:accuracy}
\end{theorem}

Our proof technique is an adaptation of the game-theoretic analysis of internal regret from the setting of online sequential classification \citep{cesa-bianchi_prediction_2006, kuleshov_estimating_2017}, and does not assume independence between the observations.

\begin{proof} 
For $Y, \bX \sim \Fbb(Y, \bX)$, denote $l(Y, F)(t)= L(Y, F(t|\bX))$ the accuracy measure that involves the observation $Y$ and the corresponding predictive CDF $F(Y|\bX)$ evaluated at $t \in \Ysc$. For an observed data pair $\{y_i, \bx_i \}$, denote the corresponding empirical version of $l$ as $l_i(Y, F)(t)= L(y_i, F(t|\bx_i))$. Also denote $F_i(t)=F(t|\bX=\bx_i)$.\\

We notice below facts:
\begin{enumerate}
\item $l(Y, F)(t)$ is bounded by $B$, therefore for any predictive CDFs $F, F' \in \Fsc$, we always have:
$$l(Y, F)(t) - l_i(Y, F')(t) \leq B$$
\item Since $l(Y, F)(t)$ is proper in the sense that this loss is minimized by the true model parameters, then for $Y \sim \Fbb$:
$$\Fbb(t) \in
 \underset{F \in \Fsc}{argmin} \; 
E_{Y \sim \Fbb} \Big( l(Y, F)(t) \Big)
$$

\item $\bbI \Big( \hat{F}_i(t) = p_i \Big) = 
\bbI \Big( \hat{F}_i(t) = p_i, y_i < t \Big) + 
\bbI \Big( \hat{F}_i(t) = p_i, y_i > t \Big)$. \\
Furthermore,
\begin{align*}
\bbI \Big( \hat{F}_i(t) = p_i, y_i < t \Big) &=
\bbI \Big( \hat{F}_i(t) = p_i \Big) * 
\Big( \bbI \big( y_i < t | \hat{F}_i(t) = p_i \big) -  p_i \Big) + 
\bbI \Big( \hat{F}_i(t) = p_i \Big) * p_i
\\
\bbI \Big( \hat{F}_i(t) = p_i, y_i > t \Big) &=
\bbI \Big( \hat{F}_i(t) = p_i \Big) * 
\Big( p_i - \bbI \big( y_i < t | \hat{F}_i(t) = p_i \big)\Big) + 
\bbI \Big( \hat{F}_i(t) = p_i \Big) * 
\Big( 1 - p_i \Big)
\end{align*}
which implies:
$$\bbI \Big( \hat{F}_i(t) = p_i \Big) 
\leq 
2 * \bbI \Big( \hat{F}_i(t) = p_i \Big) * 
\Big| \bbI \big( y_i < t | \hat{F}_i(t) = p_i \big) -  p \Big| + 
\bbI \Big( \hat{F}_i(t) = p_i \Big) * p_i(t)
$$
where $p_i(t) = p_i$ if $y_i < t$ and $p_i(t) = 1 - p_i$ otherwise.
\end{enumerate}
Combining above facts, we have:
\begin{align}
\bbL(Y, \hat{F})(t) - \bbL(Y, \hat{F}_0)(t) 
&=
\frac{1}{N} \sum_{i=1}^N
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * \bbI(\hat{F}_i(t)=p_i) 
\nonumber \\
&\leq 2 \frac{1}{N} \sum_{i=1}^N 
\underline{\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big)} * 
\Big| \bbI \big( y_i < t | \hat{F}_{i}(t) = p_i \big) -  p_i \Big|  * 
\bbI(\hat{F}_i(t)=p_i)  + 
\nonumber \\
& \qquad \frac{1}{N}\sum_{i=1}^N  
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * 
p_i(t) * 
\bbI(\hat{F}_i(t)=p_i) 
\nonumber \\
&\leq 2B * \bigg\{
\frac{1}{N} \sum_{i=1}^N 
\Big| \bbI \big( y_i < t | \hat{F}_{i}(t) = p_i \big) -  p_i \Big| * 
\bbI(\hat{F}_i(t)=p_i) 
\bigg\}
\; + 
\nonumber \\
& \qquad \bigg\{ 
\frac{1}{N}\sum_{i=1}^N  
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * 
p_i(t) * 
\bbI(\hat{F}_i(t)=p_i) \bigg\}
\label{eq:proof_part1}
\end{align}
Here the first inequality uses Fact 3. The second inequality uses  Fact 1 on the underlined component.

We now consider the two expressions in curly brackets in (\ref{eq:proof_part1}). Notice the first expression corresponds to an "unintegrated" version of calibration loss:
\begin{align}
\frac{1}{N} \sum_{i=1}^N 
\Big| \bbI \big( y_i < t | \hat{F}_{i}(t) = p_i \big) -  p_i \Big| * 
\bbI(\hat{F}_i(t)=p_i) 
& = 
 \frac{1}{N} \sum_{i=1}^N 
\Big| \bbI \big( y_i < t | \bx_i \big) -  \hat{F}_{i}(t) \Big| 
= \bbC(Y, \hat{F})(t),
\label{eq:exp_1}
\end{align}
and the second expression can be written as:
\begin{align}
& \quad \frac{1}{N}\sum_{i=1}^N  
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * 
p_i(t) * \bbI(\hat{F}_i(t)=p_i) 
\nonumber\\
& =
\frac{1}{N} \bigg[
\sum_{y_i < t}
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * \hat{F}_i(t) + 
\sum_{y_i \geq t}
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * (1 - \hat{F}_i(t))
\bigg]
\nonumber\\
& \leq
\frac{1}{N} \bigg[
\sum_{y_i < t}
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * \bbI\big( y_i < t | \bx_i \big) + 
\sum_{y_i \geq t}
\Big( l_i(Y, \hat{F})(t) - l_i(Y, \hat{F}_0)(t) \Big) * \bbI\big( y_i > t | \bx_i \big)
\bigg] + \epsilon_n
\nonumber\\
& = \mathbb{E}
\Big( l(Y, \hat{F})(t) - l(Y, \hat{F}_0)(t) \Big) + \epsilon_n 
\nonumber\\
& \leq 
\mathbb{E}
\Big( l(Y, \Fbb)(t) - l(Y, \hat{F}_0)(t) \Big) + (B + 1)\epsilon_n 
\nonumber\\
& \leq (B + 1)\epsilon_n
\label{eq:exp_2}
\end{align}
where the first inequality follows since $\hat{F}$ is $\epsilon_n$-calibrated, the second inequality follows since $l$ is a bounded loss, and the last inequality follows since $l$ is a proper loss.

Now replace the two expressions within brackets in (\ref{eq:proof_part1}) with (\ref{eq:exp_1}) and (\ref{eq:exp_2}), we have:
\begin{align*}
\bbL(Y, \hat{F})(t) - \bbL(Y, \hat{F}_0)(t) 
& \leq 2B * \bbC(Y, \hat{F})(t) + (B + 1)\epsilon_n
\end{align*}
Intergrating both sides of above equation with respect to $t \in \Ysc$, we have:
$$\bbL(Y, \hat{F}) - \bbL(Y, \hat{F}_0) \leq 2B * \bbC(Y, \hat{F}) + (B + 1)\epsilon_n$$
\end{proof}

Notice that Theorem \ref{thm:accuracy} is applicable to most of the standard measures for predictive accuracy, e.g. root mean squared error (RMSE). This is because for suitably standardized $\{y_i\}_{i=1}^N$, RMSE is always  bounded and proper \citep{gneiting_strictly_2007}. 

==> sections/proof/bne_mean.tex <==
Recall the ``Darth Vadar rule" \citep{muldowney_darth_2012}:
\begin{align}
E(s(y)|\bx) &= \int_{y \in \Ysc} 
\deriv{y}s(y) * \big[ I(y>0) - F(y|\bx) \big] dy
\label{eq:darth}
\end{align}
Also recall that \gls{BNE}'s model \gls{CDF} is $F(y|\bx, G, \Phi) = G \Big[ F_S(y|\bx, \Phi) \Big]$. Therefore we can expresse the predictive mean $E(y|\bx, G, \Phi)$ for full \gls{BNE} in terms of its CDF:
\begin{align*}
E(y|\bx, G, \Phi)
&= \int_{y \in \Ysc} I(y>0) - F(y|\bx, G, \Phi) dy\\
&= \int_{y \in \Ysc} I(y>0) - G \Big[ F_S(y|\bx, \Phi) \Big] dy \\
&= \int_{y \in \Ysc} 
\Big[ I(y>0) - F_S(y|\bx, \Phi) \Big] + 
\Big[ F_S(y|\bx, \Phi) - G \big[ F_S(y|\bx, \Phi) \big] \Big] dy \\
&= \underline{\int_{y \in \Ysc} 
\Big[ I(y>0) - F_S(y|\bx, \Phi) \Big] dy} + 
\int_{y \in \Ysc} 
\Big[ F_S(y|\bx, \Phi) - G \big[ F_S(y|\bx, \Phi) \big] \Big] dy
\end{align*}
Notice in the last line of above expression, the first integral (underlined) is the predictive mean with respect to the additive ensemble model $Y=\sum_{k=1}^K f_k(\bx)\mu_k + \delta(\bx) + \epsilon$. Therefore:
\begin{align}
E(y|\bx, G, \Phi) &= 
\sum_{k=1}^K f_k(\bx)\mu_k + 
\underbrace{\delta(\bx)}_{D_\delta(y|\bx)} + 
\underbrace{\int_{y \in \Ysc} 
\Big[ F_S(y|\bx, \Phi) - G \big[ F_S(y|\bx, \Phi) \big] \Big] dy}_{D_G(y|\bx)} \nonumber 
\\
&= \sum_{k=1}^K f_k(\bx)\mu_k + D_\delta(y|\bx) + D_G(y|\bx)
\label{eq:mean_decomp}
\end{align}


==> sections/proof/pdf.tex <==
\begin{proof}
To derive the expression of PDF in (\ref{eq:cpg_pdf}), only need to derive the constant term $C$ by integrating over \gls{CGP}'s unnormalized likelihood function in (\ref{eq:cgp_cond_lkhd}):
\begin{alignat}{3}
    C 
    &= \int_{\bg \in \real^n} \Phi(\bA \bg + \bb) * \phi(\bg |\bu,  \bK) d\bg 
    \nonumber\\
    &= P \big( \bZ \leq \bA \bg + \bb \big)  \qquad 
    &&\mbox{where}\quad 
    \bZ \sim \phi(0, \bI)
    \nonumber\\
    &= P \big( \bZ \leq \bA(\bGamma \bZ' + \bu) + \bb \big)  \qquad 
    &&\mbox{where}\quad 
    \bZ' \sim \phi(0, \bI), \bZ' \indep \bZ, \bA=\bGamma\bGamma^\top 
    \nonumber\\
    &= P \big( \bZ - \bA\bGamma \bZ' \leq \bA\bu + \bb \big)  \qquad 
    &&\mbox{notice}\quad 
    \bZ - \bA\bGamma \bZ' \sim \phi(0, \Sigma=\bI + \bA\bK\bA^\top)
    \nonumber\\
    &= \Phi(\bA\bu + \bb|\bSigma=\bI + \bA\bK\bA^\top)
    \label{eq:cdf_integral}
\end{alignat}
Now derive the expression for \gls{MGF}:
\begin{alignat*}{3}
    M_{\bg}(\bt) 
    &= E(exp(\bt^\top \bg )|\Csc, \bu, \bK) \\
    &= \int_{\bg \in \real^n}
    exp(\bt^\top \bg ) * \phi(\bg |\bu,  \bK) * \Phi(\bA \bg + \bb)d\bg /C  \\
    &\propto \int_{\bg \in \real^n} 
    exp(- \frac{1}{2} \bg \bK^{-1} \bg + (\bK^{-1}\bu + \bt)^\top\bg ) * \Phi(\bA \bg + \bb)  d\bg /C 
    \qquad &&\mbox{complete square in exp term}
    \\
    &= \int_{\bg \in \real^n} 
    exp(\bu^\top\bt + \frac{1}{2} \bt^\top \bK \bt ) * 
    \phi(\bg|\mu = \bu + \bK\bt, \Sigma=\bK) * \Phi(\bA \bg + \bb)  d\bg /C
    \\
    &= exp(\bu^\top\bt + \frac{1}{2} \bt^\top \bK \bt ) * 
    \int_{\bg \in \real^n} 
    \phi(\bg|\mu = \bu + \bK\bt, \Sigma=\bK) * \Phi(\bA \bg + \bb) d\bg  /C
    \qquad &&\mbox{compute integration as in (\ref{eq:cdf_integral})}
    \\
    &= exp(\bu^\top\bt + \frac{1}{2} \bt^\top \bK \bt ) * 
    \Phi(\bA(\bu + \bK\bt) + \bb | \Sigma = \bI + \bA\bK\bA^\top)/C
    \qquad &&\mbox{plug in expression of $C$}
    \\
    &= exp(\bu^\top\bt + \frac{1}{2} \bt^\top \bK \bt ) * 
    \frac{
    \Phi(\bA\bu + \bb + \bA\bK\bt |\Sigma = \bI + \bA\bK\bA^\top)}{
    \Phi(\bA\bu + \bb|\Sigma = \bI + \bA\bK\bA^\top)}
\end{alignat*}
\end{proof}

